Sub-Turing Islands in the Wild

Recently, there has been growing debate as to whether or not static analysis can be truly sound. In spite of this concern, research on techniques seeking to at least partially answer undecidable questions has a long history. However, little attention has been given to the more empirical question of how often an exact solution might be given to a question despite the question being, at least in theory, undecidable. This paper investigates this issue by exploring sub-Turing islands -- regions of code for which a question of interest is decidable. We define such islands and then consider how to identify them. We implemented Cook, a prototype for finding sub-Turing islands and applied it to a corpus of 1100 Android applications, containing over 2 million methods. Results reveal that 55\% of the all methods are sub-Turing. Our results also provide empirical, scientific evidence for the scalability of sub-Turing island identification. Sub-Turing identification has many downstream applications, because islands are so amenable to static analysis. We illustrate two downstream uses of the analysis. In the first, we found that over 37\% of the verification conditions associated with runtime exceptions fell within sub-Turing islands and thus are statically decidable. A second use of our analysis is during code review where it provides guidance to developers. The sub-Turing islands from our study turns out to contain significantly fewer bugs than `theswamp' (non sub-Turing methods). The greater bug density in the swamp is unsurprising; the fact that bugs remain prevalent in islands is, however, surprising: these are bugs whose repair can be fully automated.

==> oracles.tex <==
\section{Oracle Realization: Loop Summaries}
\label{sec:loop_summaries}
As part of this section, we present a realization of the oracle $O_s$ capable of answering if a summary is computable for a given loop with respect to a given set of variables. But the existence of the  summary is not enough. Indeed, the summary itself is required for our analysis (section~\ref{sec:identify_st-islands}). Therefore, we also cover the computation of summaries. For this, we provide a lightweight algorithm based on syntactic matching for inferring loop functions. As the form of loops varies a lot, it will be inefficient to perform the matching at the control-flow graph level due to irrelevant details carrying noise and preventing generalization. Hence, we need to introduce a kind of canonization to get as close to the semantics as possible. It simply consists of considering the path formula of each cycle instead of the cycle of the loop itself. We first introduce some pre-required material.

\subsection{Program Representaion}
For the sake of formal reasoning, let us assume that a program is represented in terms of transition constraints over unprimed and primed variables including the program counter ($pc$). Primed variables refer to the transition post-state while unprimed ones refer to the pre-state. Such a representation can be easily extracted from the program control flow graph. An example of a code and the corresponding set of transition constraints is given in Figure~\ref{fig:example}.  
\begin{figure*}[t]
\begin{center}
\begin{tabular}{c@{\hspace{1in}}c}
\hline
\\
\begin{minipage}{4cm}
\begin{lstlisting}
int i = 0;
int j = 0;
while (i < n){
	i = i + 1;
	j = j + 3;
}
\end{lstlisting}

\iffalse
\begin{verbatim}
1:  int i = 0;
2:  int j = 0;
  
3:  while (i < n)
    {
4:      i = i + 1;
5:      j = j + 3;
6:  }
\end{verbatim}
\fi

\end{minipage}
&
\begin{tabular}{l}
$pc=1 \wedge i' = 0 \wedge pc'=2 $\\
$pc=2 \wedge j' = 0 \wedge pc'=3 $\\
$pc=3 \wedge i < n \wedge pc'=4 $\\
$pc=3 \wedge i \geq n \wedge pc'=6 $\\
$pc=4 \wedge i' = i + 1 \wedge pc'=5 $\\
$pc=5 \wedge j' = j + 3 \wedge pc'=3 $\\
\end{tabular}
\\
\\
(a) & (b)
\\
&
\\
\hline

\end{tabular}
\caption{A simple program (a) and the corresponding set of transition constraints (b).}
\label{fig:example}
\end{center}
\end{figure*}

Unprimed conjuncts are called guards and primed ones are called updates. Hence, for a transition $\tc$, we write $\tc \equiv pc = \ell \wedge \pi \wedge u \wedge pc'= \ell'$, where $\pi$ is the conjunction of all guards, except the one over $pc$, and $u$ is the conjunction of all updates, excluding the assignment to $pc$. We write $\pi(\tc)$ to refer to the guard of $\tc$ and $u(\tc)$ to refer to its update.

\subsection{Transition Composition}
Transitions are either primitive or resulting from the compositions of other transitions. Given two transition constraints $\tc_1 \equiv G_1 \wedge X' = E_1$ and $\tc_2 \equiv G_2 \wedge X' = E_2$, their composition is 
\begin{equation}
\exists Y.\; \tc_1[Y/X'] \wedge \tc_2[Y/X]
\label{eq:transcomp}
\end{equation}

\iffalse
\begin{equation}
\tc_1 \circ \tc_2 = G_1 \wedge \tc_2[E_1/X]
\label{eq:transcomp}
\end{equation}
\fi
\iffalse
\begin{exmp}
Consider the list of transition constraints below:
\[
\begin{array}{ll}
\tc_1: & pc=1 \wedge x > 0 \wedge pc'=2 \\
\tc_2: & pc=2 \wedge y' = x + 1 \wedge pc'=3 \\
\tc_3: & pc=3 \wedge y > 2 \wedge pc'=4 \\
\tc_4: & pc=4 \wedge z' = y \wedge pc'=5 \\
\end{array}
\] 
The composition of $\tc_1$ and $\tc_2$ gives 
\[
\tc_1 \circ \tc_2 \equiv  pc=1 \wedge x > 0 \wedge y' = x + 1 \wedge pc'=3
\]
Composing the previous result with $\tc_3$  gives
\[
pc=1 \wedge x > 0 \wedge x +1 > 2 \wedge y' = x + 1 \wedge pc'=4
\]
Finally, the composition of the last formula with $\tc_4$ results in
\[
pc=1 \wedge x > 0 \wedge x +1 > 2 \wedge y' = x + 1 \wedge z' = x + 1 \wedge pc'= 5
\]
In the final formula, we have
\[
g \equiv x > 0 \wedge x +1 > 2
\] 
and 
\[
u \equiv y' = x + 1 \wedge z' = x + 1
\]
\end{exmp}
\fi
\begin{definition} [Path Formula]
Given a transition path $\tc_1,\ldots,\tc_{k}$, the corresponding \emph{path formula} is given by  
\[
\pathform(\tc_1,\ldots,\tc_{k}) = \tc_1 \circ\ldots \circ\tc_{k}
\]	 
It represents the composition of all transitions forming the path. \end{definition}
From the definition of transition constraints and their composition, a path formula is always a conjunction of atomic predicates, i.e., connector-free predicates. Given a path formula $\varphi$, we write $a(\varphi)$ to denote the set of atomic predicates appearing in it.   

\subsection{Loops and Cycles} 
Answering whether a summary for a given a loop is computable is in general undecidable. We are interested in subset of loops for which that question is decidable that we call \emph{sub-Turing} loops or simply \emph{ST-loops}. To start with, an ST-loop $\myloop$ is a set of cycles $\cycle_1,\ldots,\cycle_k$, such that each cycle $\cycle_i$ ($i \in [1..k]$) has the form
\[
\cycle_i \equiv pc = \ell_H \wedge \pi_i \wedge u_i \wedge pc' = \ell_H
\]
were $\ell_H$ is the location of the header of the loop $\myloop$.  We assume absence of non-determinism. Hence, guards of any two cycles $\cycle_i$ and $\cycle_j$ ($i,j \in [1..k]$) are mutually exclusive, i.e., $\pi_i \wedge \pi_j \equiv \false$. 

The path formula for $\myloop$ is 
\[
\pathform(\myloop) \equiv \bigvee_{i \in [1..k]} \pathform(\cycle_i)
\]



\subsection{Term Types}
We introduce the notion of term types that we use later in the presentation. 

\begin{definition}[Counter]
A variable is a counter if it is incremented by a constant amount within a cycle. Formally speaking, a variable $j$ is a counter if
\begin{align*}
\forall \cycle \in \myloop.\;\;(\cycle \myimplies j' = j + d_\cycle) \vee (\cycle \myimplies j' = j) \;
\\
\text{s.t.\; $d_\cycle$ is constant.}
\end{align*}
We use $CT(\myloop)$ to denote the set of counters in a loop $\myloop$. 
\end{definition}
\begin{definition}[Induction Variable]
An induction variable is a counter that is incremented by one at each iteration of $\myloop$. More precisely, we say that $i$ is an induction variable for the loop $\myloop$ if  
\[
\myloop \myimplies i' = i + 1
\]  
We use $i$ to refer to the loop induction variable. Where more than one induction variable exists, we arbitrarily select one. 
\end{definition}
\begin{Remark}
The constraint of the induction variable stride to be 1 is to ease the presentation. If the stride is a constant different from 1, we can rewrite it in terms of another induction variable, with 1 as stride, that we freshly introduce.     
\end{Remark}
\begin{definition}[I-Indexed Write Array]
An i-indexed write array $a$ is an array that is updated through the loop induction variable $i$ as index. We write $\mathit{WR}(\myloop)$ to refer to the set of write arrays in the loop $\myloop$. Formally speaking, $a$ is a write array if
\begin{align*}
\forall \cycle \in \myloop.\;\;(\cycle \myimplies a'[i] = e) \vee (\cycle \myimplies a'[i] = a[i])
\\
\text{ \;\;s.t.\;\;} (CT(\myloop) \cup \mathit{WA}(\myloop)) \cap var(e) = \phi.
\end{align*}

In the formula above $e$ is an expression and $var(e)$ (as previously) is the set of identifiers (symbols) appearing in it. Hence, the only variable updated inside the loop that can appear in $e$ is $i$. 
\end{definition}
\begin{Remark}
We handle other data structures, such as collections, by modelling them as arrays.   
\end{Remark}
\begin{definition}[Induction guard]
An induction guard $\varphi$ is an unprimed predicate appearing in a cycle $\cycle \in \myloop$ such that
\[var(\varphi) \cap (CT(\myloop) \cup WA(\myloop)) = \phi.\] 
We write $IG(\myloop)$ to denote the set of induction guards. 
\end{definition}

\subsection{Summary Inference for ST-Loops}
Given a loop $\myloop$, we want to infer for program variables expressions modelling their after-values with respect to the execution of $\myloop$. If we are able to infer such expressions for all variables, we say that $\myloop$ is an ST-loop. 

A main challenge in reasoning about loops is dependencies between statements at different iterations known as loop-carried dependencies. A second challenge is due to the presence of multiple cycles as  we need to account for all (possibly infinite) number of interleavings between them. To overcome these issues, we propose a set of syntactic constraints enabling us to rule out loop-carried dependencies while performing a modular reasoning. Loops obeying our constraints are instances of ST-loops that we call \emph{dependency-free}.

\begin{definition}[Dependency-free Loops]
A loop $\myloop$ is dependency-free and thus sub-Turing if for any cycle $\cycle \in \myloop$ we have
\begin{enumerate}
\item For any update in $a(u(\cycle))$ of the form $x' = e$, ${x \in CT(\myloop)}$
\item For any update in $a(u(\cycle))$ of the form $a'[i] = e$, ${a \in \mathit{WA}(\myloop)}$ 
\item For any guard $\varphi \in a(\pi(\cycle))$, $\varphi \in IG(\myloop)$
\end{enumerate} 
For a loop $\myloop$, we write $DF(\myloop)$ to indicate that it fulfils constraints (1), (2) and (3).
\end{definition}

As you can see from constraints (1) and (2), the only kind of updates allowed inside a cycle are i-indexed write arrays and counters. I-indexed write arrays ensure that each array element is written once and its index  only depends on the induction variable $i$. Counters have the property that their final values only depend on the number of increments associated with each constant. Constraint (3) ensures that no cycle has any effect on the remaining ones. As a consequence, we can reason about each cycle individually. The result is then combined to form a summary  for the loop. 

Hence a realization for the oracle $O_s$ is simply a test if $DF(\myloop)$ holds for the loop taken as parameter. In what follows, we proof by construction the existence of a summary for a loop $\myloop$ if the constraints expressed by $DF(\myloop)$ are met. 

\begin{proposition}
A summary is always inferable for a loop $\myloop$ if $DF(\myloop)$ holds. 
\end{proposition}

\begin{Sketch}
To prove the proposition above we construct a summary and prove its correctness. We reason about i-indexed write arrays and counters separately. For each case, we apply induction on the number of iteration of a given loop. At each iteration any cycle can be executed. By inferring a formula describing modified arrays and another one describing counters, their conjunction is the summary for the loop. Therefore the loop is sub-Turing.  

 
\end{Sketch}
\subsection{Summary for Counters} 

Given a counter $m$ and a set of cycles $\cycle_j \in \myloop$ ($j \in J$) where $m$ is modified, we propose the rule \textsc{counter}, in Figure~\ref{fig:rules}(a), to infer the post-state value of counter $m$ with respect to $\myloop$. Function $\mathsf{num}(\varphi(x),k,l)$, used in the rule, returns the number of elements in the interval $[k..l]$ for which $\varphi(x)$ is true.
\begin{figure*}
\begin{center}
\begin{minipage}{12cm}
\begin{tabular}{|@{\hspace{-1cm}}c|}
\hline
\\
\begin{mathpar}
\inferrule* [Right=(counter)]
{DF(\myloop), \text{ for } j \in J.\; \cycle_j \in \myloop \wedge \cycle_j \myimplies m' = m + d_J}{m' = m + \sum_{j \in J} d_j * \mathsf{num}(\cycle_j.\pi[x/i],i,i'-1) 
}
\end{mathpar}
\\
(a)
\\
\\
\\
\begin{mathpar}
\inferrule* [Right=(write-array)]
{DF(\myloop), \text{ for } j \in J.\; \cycle_j \in \myloop \wedge \cycle_j \myimplies a'[i] = e_j}{\forall j \in J \; \forall x \in [i..i'-1].\; \cycle_j.\pi[x/i] \myimplies a'[x] = e_j}
\end{mathpar}
\\
\\
(b)
\\
\hline
\end{tabular}
\end{minipage}
\end{center}
\caption{Inference rules for summarising counter variables (a) and arrays (b).}
\label{fig:rules}
\end{figure*}




\begin{proposition}[Rule counter]
The formula inferred by rule \textsc{counter} applied to a loop $\myloop$ and a counter $m$ exactly expresses the symbolic value of $m$ after an arbitrary number of iterations of $\myloop$.
\end{proposition}
\begin{proof}
We prove the previous proposition by induction on the number of iterations of loop $\myloop$. 

For the basic case, we assume that $\myloop$ is executed once. Hence, one cycle $\cycle_k \in \myloop$ is executed. Therefore $\cycle_k.\pi$ is true. We have
\[\cycle_k \myimplies m' = m + d_k\]
As $\cycle_k.\pi$ holds for $i$, it means that $\mathsf{num}(\cycle_k.\pi,i,i) = 1$, which can be rewritten to $\mathsf{num}(\cycle_k.\pi,i,i-1) = 1$  as $i' = i + 1$. Hence we have
 \[\cycle_k \myimplies m' = m + d_k * \mathsf{num}(\cycle_k.\pi,i,i-1)\]
For all other cycles $\cycle_l$ ($l \neq k$), $\cycle_l.\pi$ is false, implying $\mathsf{num}(\cycle_l.\pi,i,i'-1) = 0$. As a result we have  
\[\cycle_k \myimplies m' = m + \sum_{j \in J} d_j * \mathsf{num}(\cycle_j.\pi[x/i],i,i'-1)\]
or 
\begin{equation}
\pathform(\myloop) \myimplies m' = m + \sum_{j \in J} d_j * \mathsf{num}(\cycle_j.\pi[x/i],i,i'-1)
\label{eq:c_basic}
\end{equation}
Which correspond to the result of rule \textsc{counter}.

Now we prove the induction step. We assume 
\[\pathform(\myloop)^{\langle n\rangle} \myimplies m' = m + \sum_{j \in J} d_j * \mathsf{num}(\cycle_j.\pi[x/i],i,i'-1)\]
and we try to prove 
\begin{equation}
\pathform(\myloop)^{\langle n+1\rangle} \myimplies m' = m + \sum_{j \in J} d_j * \mathsf{num}(\cycle_j.\pi[x/i],i,i'-1).
\label{eq:c_target}
\end{equation}
We have 
\[\pathform(\myloop)^{\langle n+1\rangle} = \pathform(\myloop)^{\langle n\rangle} \circ \pathform(\myloop)\]
Hence 
\begin{align*}
\pathform(\myloop)^{\langle n+1\rangle} \myimplies
\\
 (m' = m + \sum_{j \in J} d_j * \mathsf{num}(\cycle_j.\pi[x/i],i,i'-1)) \circ \pathform(\myloop)
\end{align*}

By using the result of (\ref{eq:c_basic}), we obtain
\begin{align*}
\pathform(\myloop)^{\langle n+1\rangle} \myimplies
\\
 ((m' = m + \sum_{j \in J} d_j * \mathsf{num}(\cycle_j.\pi[x/i],i,i'-1)) 
\\ 
 \circ (m' = m + \sum_{j \in J} d_j * \mathsf{num}(\cycle_j.\pi[x/i],i,i'-1)))
\end{align*} 
We introducing the intermediary (fresh) variables $i''$ and $m''$ to perform the composition according to (\ref{eq:transcomp}), we obtain
\begin{align*}
\pathform(\myloop)^{\langle n+1\rangle} \myimplies
\\
 ((m'' = m + \sum_{j \in J} d_j * \mathsf{num}(\cycle_j.\pi[x/i],i,i''-1)) 
 \\
 \wedge (m' = m'' + \sum_{j \in J} d_j * \mathsf{num}(\cycle_j.\pi[x/i],i'',i'-1)))
\end{align*}
By replacing $m''$ in the right conjunct using the equality from  the left conjunct, we get
\begin{align*}
\pathform(\myloop)^{\langle n+1\rangle} \myimplies
\\
 (m' = m + \sum_{j \in J} d_j * ((\mathsf{num}(\cycle_j.\pi[x/i],i,i''-1) 
\\ 
 + \mathsf{num}(\cycle_j.\pi[x/i],i'',i'-1)))
\end{align*}
Finally, simplifications yield   
\[\pathform(\myloop)^{\langle n+1\rangle} \myimplies m' = m + \sum_{j \in J} d_j * \mathsf{num}(\cycle_j.\pi[x/i],i,i'-1)\]
Which is our target (\ref{eq:c_target}).
\end{proof}
\subsection{Summary for Arrays} 

Given a set of cycles $\cycle_j \in \myloop$ ($j \in J$) where array $a$ is updated, we propose the rule \textsc{write-array}, in Figure~\ref{fig:rules}(b), to infer the post-state value of $a$ with respect to $\myloop$.

\begin{proposition}[Rule write-array]
The formula inferred by rule \textsc{array-write} applied to a loop $\myloop$ and an array $a$ exactly expresses the symbolic value of $a$ after an arbitrary number of iterations of $\myloop$.
\end{proposition}
\begin{proof}
Similar to the case of counters, here also we use induction on the number of loop iterations to prove the proposition above. 

For the basic case,we assume that $\myloop$ is executed once. Hence, one cycle $\cycle_k \in \myloop$ is executed. Therefore $\cycle_k.\pi$ is true. We have
\[\cycle_k \myimplies \cycle_k.\pi \wedge a'[i] = e_k\]
Hence 
\[\cycle_k \myimplies (\cycle_k.\pi \myimplies a'[i] = e_k)\]
Further,
\[\cycle_k \myimplies (\forall x \in [i..i].\; \cycle_k.\pi[x/i] \myimplies a'[x] = e_k)\]
As $i' = i -1$, we obtain 
\[\cycle_k \myimplies (\forall x \in [i..i'-1].\; \cycle_k.\pi[x/i] \myimplies a'[x] = e_k)\]
Knowing that $\cycle_k.l$ is false for $l \neq k$, we can write 
\[\cycle_k \myimplies (\forall  j \in J \;\;\forall x \in [i..i'-1].\; \cycle_k.\pi[x/i] \myimplies a'[x] = e_j)\]
Finally 
\begin{equation}
\begin{split}
\pathform(\myloop) \myimplies (\forall  j \in J \;\;\forall x \in [i..i'-1].\; \cycle_k.\pi[x/i] 
\\
\myimplies a'[x] = e_j)
\end{split}
\label{eq:a_basic}
\end{equation}

Now we prove the induction step. We assume  
\begin{align*}
\pathform(\myloop)^{\langle n\rangle} 
\myimplies (\forall  j \in J \;\;\forall x \in [i..i'-1].\; \cycle_k.\pi[x/i] 
\\
\myimplies a'[x] = e_j)
\end{align*}
and try to prove 
\begin{equation}
\begin{split}
\pathform(\myloop)^{\langle n+1\rangle} \myimplies (\forall  j \in J \;\;\forall x \in [i..i'-1].\; \cycle_k.\pi[x/i] 
\\
\myimplies a'[x] = e_j)
\end{split}
\label{eq:a_target}
\end{equation}
We have 
\[\pathform(\myloop)^{\langle n+1\rangle} = \pathform(\myloop)^{\langle n\rangle} \circ \pathform(\myloop)\]
Hence
\begin{align*}
\pathform(\myloop)^{\langle n+1\rangle} \myimplies
 (\forall  j \in J \;\;\forall x \in [i..i'-1].\; \cycle_k.\pi[x/i] 
\\ 
 \myimplies a'[x] = e_j) \circ \pathform(\myloop)
\end{align*}
By using the result of (\ref{eq:a_basic}) and introducing the fresh variable $i''$ for composition according to (\ref{eq:transcomp}), we obtain
\begin{align*}
\pathform(\myloop)^{\langle n+1\rangle} \myimplies (\forall  j \in J \;\;\forall x \in [i..i''-1].\; \cycle_k.\pi[x/i] 
\\
\myimplies a'[x] = e_j) \wedge (\forall  j \in J \;\;\forall x \in [i''..i'-1].\; \cycle_k.\pi[x/i] 
\\
\myimplies a'[x] = e_j)
\end{align*}

which is rewritten to
\begin{align*}
\pathform(\myloop)^{\langle n+1\rangle} \myimplies (\forall  j \in J \;\;\forall x \in [i..i'-1].\; \cycle_k.\pi[x/i] 
\\
\myimplies a'[x] = e_j)
\end{align*}
corresponding to our target (\ref{eq:a_target}).

\end{proof}

